Black-box Membership Inference Attacks on the Pre-training Data of Image-generation Models

The rapid advancement of diffusion-based image generation models has raised serious concerns regarding potential copyright and privacy infringements involving human-created data. Membership inference attacks (MIAs) have emerged as a promising tool for identifying unauthorized data usage during model training. Existing methods typically assess the ability of model to denoise perturbed suspect images as an indicator of membership status. However, the discriminative power of such features is highly dependent on the degree of model memorization and deteriorates significantly when applied to less exposed data (e.g., pre-training data). Although several methods attempt to enhance detection by leveraging internal model features, these features are generally inaccessible in mainstream closed-source image generation platforms, limiting their practicality. In this paper, we demonstrate that analyzing how a black-box diffusion model denoises a target image and corresponding perturbed textual instructions can reveal more distinctive membership cues. Based on this insight, we propose a black-box membership inference attack framework (named SD-MIA) that leverages a cross-modal data perturbation mechanism to detect pre-training data in diffusion models. We conduct extensive experiments on both a public benchmark dataset and a newly constructed dataset, each comprising pre-training membership and non-membership samples with identical distributions. Experimental results demonstrate that SD-MIA achieves superior performance compared to existing baselines, including those with the unfair advantage of accessing internal model features.

==> sec/method.old.tex <==
\section{Methodology}
\label{sec:method}
% \subsection{Methodology Overview}
% 暂时有一点长
% Diffusion models implicitly learn a cross-modal mapping between textual descriptions and their corresponding visual representations. For training samples (members), this mapping tends to be highly localized and overfitted to the specific semantic content of the textual description $c$ and its paired image $x$. Consequently, perturbations to the textual input, such as synonym substitution, stylistic shifts, or paraphrasing, produce only minor variations in the generated image. This invariance reflects the model’s memorization of cross-modal associations between linguistic semantics and visual concepts. In contrast, for non-member pairs, the conditional distribution $p_\theta(x \mid c)$ is less concentrated, so even semantically consistent perturbations to $c$ often lead to visually divergent generations.

\begin{figure*}[t]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=1\linewidth]{fig/method.pdf}
   \caption{
   The framework of the proposed black-box MIA method SD-MIA.
   }
   \label{fig:method}
\end{figure*}

\subsection{Motivation of SD-MIA}

To determine whether a suspected image appeared in the pre-training corpus of a black-box image generative model, an intuitive strategy is to extend membership-inference techniques originally developed for fine-tuning data. 
However, our empirical evaluation shows that extensions of many these methods fail to generalize.
Their central limitation is a dependence on image-space perturbation and denoising-response analysis. 
In modern diffusion-based generators, input images are first encoded into variational latents that aggressively compress fine-grained structure and smooth away moderate perturbations. These latents then traverse a stochastic diffusion trajectory, where injected noise easily dominates any residual variation. 
As a result, perturbations applied in the image domain rarely survive the generative process, causing member and non-member samples to exhibit similarly stable reconstructions. 
Formally, let $c$ be a textual description and $x$ a target image. Consider the change in the generation probability $p(x | c;\theta^*)$ when perturbing $x$ by $\delta x$. Writing $\mathbf{z}=f_v(x)$ for the VAE encoding and $\mathbf{c}=f_e(c)$ for the text embedding, and $\theta^*$ for model parameters, the induced variation $\delta_x p$ satisfies
\begin{equation}
\begin{aligned}
   \delta_x p
   % &= \lVert p(x+\delta x | c;\theta^*) - p(x | c;\theta^*) \rVert_2 \\
   &\approx \lvert \nabla_{\mathbf{z}} p(\mathbf{z},\mathbf{c};\theta^*) \cdot \delta\mathbf{z} \rvert
   \le \lVert\nabla_{\mathbf{z}} p(\mathbf{z},\mathbf{c};\theta^*)\rVert_2 \lVert\delta\mathbf{z}\bigr\lVert_2 ,
\end{aligned}
\label{eq:delta_p}
\end{equation}
and by the (local) Lipschitz continuity of the VAE encoder,
\begin{equation}
    \bigl\|\delta\mathbf{z}\bigr\|_2
    = \bigl\| f_v(x+\delta x) - f_v(x) \bigr\|_2
    \le \bigl\| \nabla_x f_v(x) \bigr\|_2 \bigl\|\delta x\bigr\|_2 .
\label{eq:delta_z}
\end{equation}
Since the VAE encoder strongly contracts the local image manifold, $\|\delta\mathbf{z}\|_2$ typically approaches zero even for non-trivial $\|\delta x\|_2$. The stochastic diffusion dynamics then further attenuate the already minuscule latent variation, driving $\delta_x p$ toward zero regardless of potential differences in $\|\nabla_{\mathbf{z}} p\|$ between member and non-member cases.
Moreover, generation models typically do not exhibit strong memorization of pre-training images, and in black-box detection settings the quantity $\delta_x p$ is not directly observable. It must instead be inferred from the model’s generated outputs, an indirect estimation process that introduces additional stochastic variability. This added noise further obscures the already attenuated perturbation signal, making membership-dependent differences in $\delta_x p$ exceedingly difficult to detect.


In our paper, we argue that a cross-modal perturbation-reconstruction mechanism offers a more reliable pathway for detecting pre-training membership. 
Rather than perturbing images, we perturb the textual instructions that condition the generator and evaluate reconstruction consistency of the target image.
Crucially, diffusion-based image generation models process text and images through fundamentally different computational pathways. 
Textual instructions are mapped into representations that remain unnoised throughout generation, persisting as conditioning signals that guide the full denoising trajectory.
Moreover, during training, the model usually internalizes a locally overfitted mapping from the representation of a specific textual description, and its immediate representation neighborhood, into the visual features of a particular training sample. 
This induces a representation-region collapse, where a neighborhood of nearby text variants funnels toward a single visual mode.
Furthermore, for member data, small textual perturbations remain within this collapsed region, producing visual outputs that stay close to the memorized appearance.
For non-member data, no such collapsed structure exists, and perturbations can push the conditioning signal into genuinely distinct regions, yielding perceptibly divergent outputs. 
This structural asymmetry highlights the potential of cross-modal perturbation–reconstruction as an effective signal for detecting pre-training data in black-box image generation models.
Formally, when perturbing textual description $c$ by $\delta c$, the induced variation $\delta_c p$ satisfies
\begin{equation}
\begin{aligned}
   \delta_c p
   &\approx \lvert \nabla_{\mathbf{c}} p(\mathbf{z},\mathbf{c};\theta^*) \cdot \delta\mathbf{c} \rvert
   \le \lVert\nabla_{\mathbf{c}} p(\mathbf{z},\mathbf{c};\theta^*)\rVert_2 \lVert\delta\mathbf{c}\bigr\lVert_2 ,
\end{aligned}
\label{eq:delta_c}
\end{equation}
Under representation-region collapse, member pairs $(x_m,c_m)$ satisfy $\left\| \nabla_{\mathbf{c}} p(\mathbf{z}_m,\mathbf{c}_m;\theta^*) \right\|_2 \approx 0$, while this condition does not hold for non-member pairs $(x_n,c_n)$.
Since textual perturbations induce observable shifts $\delta\mathbf{c}$ in the embedding space, we obtain $\delta_c p(x_m) \ll \delta_c p(x_n)$ for identical perturbation magnitudes $\left\| \delta\mathbf{c} \right\|_2$, forming the theoretical basis for black-box membership inference of pre-training data via cross-modal perturbation.
We further note that this work is, to the best of our knowledge, the first to conceptualize and instantiate a cross-modal perturbation-reconstruction mechanism for membership inference, a direction not explored in prior studies.

\subsection*{Version 2}
To determine whether a suspected image appeared in the pre-training corpus of a black-box image generative model, an intuitive strategy is to extend membership-inference techniques originally developed for fine-tuning data. However, our empirical evaluation shows that many such extensions fail to generalize. Their central limitation lies in their reliance on image-space perturbation and denoising-response analysis.
In modern diffusion-based generators, input images are first encoded into variational latents that aggressively compress fine-grained structure and smooth away moderate perturbations. These latents then traverse a stochastic diffusion trajectory, where injected noise rapidly overwhelms any residual variation. As a result, perturbations applied in the image domain rarely survive the generative process, causing member and non-member samples to exhibit similarly stable reconstructions.
Formally, let $c$ be a textual description and $x$ a target image. Consider the change in the (unobservable) generation probability $p(x| c;\theta^*)$ when perturbing $x$ by $\delta x$. Writing $\mathbf{z}=f_v(x)$ for the VAE encoding, $\mathbf{c}=f_e(c)$ for the text embedding, and $\theta^*$ for model parameters, the induced variation $\delta_x p$ satisfies
\begin{equation}
\begin{aligned}
    \delta_x p
    &\approx \bigl| \nabla_{\mathbf z} p(\mathbf z,\mathbf c;\theta^*) \cdot \delta \mathbf z \bigr| \\
    &\lesssim \bigl\| \nabla_{\mathbf z} p(\mathbf z,\mathbf c;\theta^*) \bigr\|_2 \cdot \bigl\|\delta \mathbf z \bigr\|_2 .
\end{aligned}
\label{eq:delta_p}
\end{equation}
Since the VAE encoder is locally contractive, we further have
\begin{equation}
    \bigl\|\delta\mathbf z\bigr\|_2
    = \bigl\| f_v(x+\delta x) - f_v(x) \bigr\|_2
    \lesssim \bigl\| J_{f_v}(x) \bigr\|_2 \, \bigl\| \delta x \bigr\|_2 ,
\label{eq:delta_z}
\end{equation}
where $J_{f_v}(x)$ denotes the Jacobian of the encoder at $x$. Since $\|J_{f_v}(x)\|_2 \ll 1$ for typical VAEs, $\|\delta\mathbf z\|_2$ approaches zero even for non-trivial $\|\delta x\|_2$. The stochastic diffusion dynamics further attenuate this already minuscule latent variation, driving $\delta_x p$ toward zero regardless of potential differences in $\|\nabla_{\mathbf z} p\|$ between member and non-member cases. Moreover, generation models rarely memorize pre-training images strongly, and in black-box settings the quantity $\delta_x p$ is not directly observable. Any attempt to infer it from generated samples introduces additional noise, further obscuring membership-relevant differences.

In contrast, we argue that a {cross-modal perturbation--reconstruction} mechanism offers a more reliable pathway for detecting pre-training membership. Rather than perturbing images, we perturb the textual instructions that condition the generator and evaluate reconstruction consistency of the target image. Crucially, text and images follow fundamentally different computational pathways in diffusion generators: textual instructions are mapped into representations that remain unnoised throughout the entire generation process, persisting as conditioning signals that guide the denoising trajectory.
During training, the model usually internalizes a locally overfitted mapping from the representation of a specific textual description, and its immediate representation neighborhood, into the visual features of a particular training sample. This induces a {representation-region collapse}, in which a neighborhood of text variants funnels toward a single visual mode. For member data, small textual perturbations remain within this collapsed region, producing outputs that remain close to the memorized appearance. For non-member data, no such collapsed structure exists, and perturbations shift the conditioning signal into distinct regions, yielding perceptibly divergent outputs. 
Here, we give a more formal analysis: when perturbing $c$ by $\delta c$, the induced variation satisfies
\begin{equation}
\begin{aligned}
    \delta_c p
    &\approx \bigl| \nabla_{\mathbf c} p(\mathbf z,\mathbf c;\theta^*) \cdot \delta \mathbf c \bigr| \\
    &\lesssim \bigl\| \nabla_{\mathbf c} p(\mathbf z,\mathbf c;\theta^*) \bigr\|_2 \cdot \bigl\|\delta \mathbf c \bigr\|_2 .
\end{aligned}
\label{eq:delta_c}
\end{equation}
Under representation region collapse, member pairs $(x_m,c_m)$ satisfy
\[
    \bigl\| \nabla_{\mathbf c} p(\mathbf z_m,\mathbf c_m;\theta^*) \bigr\|_2 \approx 0,
\]
while this condition does not hold for non-member pairs $(x_n,c_n)$. Since textual perturbations induce observable shifts $\delta\mathbf c$ in the embedding space, we obtain
\[
    \delta_c p(x_m) \ll \delta_c p(x_n)
\]
for identical perturbation magnitudes $\|\delta\mathbf c\|_2$, forming the theoretical basis for membership inference of pre-training data via cross-modal perturbation.
We further note that , to the best of our knowledge, a cross-modal perturbation-reconstruction mechanism is not systematically  conceptualized and instantiated for membership inference, in prior studies.

In black-box settings, since $p(x\mid c;\theta^*)$ is inaccessible, we operationalize the above intuition using an observable consistency score
\[
S(x,c) \triangleq \mathbb{E}_{\varepsilon}\Bigl[ d\bigl( g(c;\varepsilon), \, x \bigr) \Bigr],
\]
where $g(c;\varepsilon)$ denotes the generator with sampling noise $\varepsilon$, and $d(\cdot,\cdot)$ is a perceptual similarity metric. Under cross-modal perturbation, we measure
\[
\delta_c S \triangleq S(x,\,c+\delta c) - S(x,\,c) ,
\]
which serves as a black-box proxy for $\delta_c p$. Our method detects membership by identifying the large-scale observed variation $\delta_c S$.


% Formally, given a pair of textual description $c$ and a target image $x$, the variation $\delta_x {p}$ of generation probability $p(x|c;\theta^*)$ of the target model $\theta^*$  resulted by perturbing the target image $x$ can be formulated as:
% \begin{equation}
% \begin{aligned}
%    \delta_c p &= || p(x+\delta x|c;\theta^*) -  p(x|c;\theta^*)||_2 \\ &\simeq |\nabla_{\theta}  p(\textbf{z},\textbf{c};\theta^*)\cdot \delta\textbf{z} |  \leq  ||\nabla_{\theta}  p(\textbf{z},\textbf{c};\theta^*)||_2 ||\delta\textbf{z} ||_2,
% \end{aligned}
% \end{equation}
% \begin{equation}
%     ||\delta\textbf{z} ||_2  =|f_v(x+\delta x)-f_v(x)| \le ||\nabla_x f_v||_2\cdot ||\delta x||_2
% \end{equation}
% where  $\textbf{z} = f_v(x)$, $f_v(\cdot)$ denotes the VAE encoder, $\textbf{c} = f_e(c)$, $f_e(\cdot)$ denotes the text embedding encoder.
% Due to the compression nature of VAE encoder, $\delta \textbf{z}$ usually tends to be zero, dominating the probability $\delta_x p$ tend to be zero no matter the potential different value of $\nabla_\theta p$ of membership and non-membership samples. 
% Thus, a model usually does not strongly memorize details of its pre-training images, making this perturbation-response signal collapse into noise.

\subsection{Cross-Modal Memorization Hypothesis}
Diffusion models are trained on large-scale collections of text–image pairs to approximate the joint distribution $p_\theta(x,c)$ over images $x$ and description $c$, thereby learning a cross-modal alignment between linguistic semantics and visual content. 
We hypothesize that for training samples, this alignment becomes locally overfitted: the diffusion model develops a strong semantic anchoring between a textual description $c$ and its corresponding image $x$, effectively reducing uncertainty in the conditional distribution. Specifically, for a member sample $(x,c)$, the conditional distribution $p_\theta(x \mid c)$ concentrates tightly around the original data manifold~\cite{ho2020denoising,carlini2019secret}, whereas for a non-member sample $(\bar{x},\bar{c})$ it remains comparatively diffuse:
\begin{equation}
\mathcal{H}\big[p_\theta(x \mid c)\big]
<
\mathcal{H}\big[p_\theta(\bar{x}\mid \bar{c} )\big],
\end{equation}
where $\mathcal{H}[ \cdot]$denotes the entropy of the conditional image distribution.
This entropy gap reflects a memorization-induced reduction of uncertainty in the denoising trajectory for seen samples in the pretraining process.
This theoretical insight motivates the design of the proposed SD-MIA framework, which probes diffusion models through controlled cross-modal perturbations to measure their semantic response sensitivity. By quantifying how invariant the generated image remains under textual variations, we extract a discriminative signal reflecting the model’s internal memorization strength for cross-modal correlation.
% To formalize the model’s response to textual perturbations, consider a  modification $\delta_c$ applied to $c$
% , resulting in a perturbed textual description $c^{'}=G( c, \delta_c)$.
% If the model has memorized the image, its generated image under the perturbation should remain highly similar to the original $x$:
% \begin{equation}
% \mathbb{E}{x' \sim p\theta(\cdot \mid c')}
% \big[
% d(\mathcal{E}_v(x'), \mathcal{E}_v(x))
% \big]
% < \varepsilon ,
% \end{equation}
% where $d(\cdot,\cdot)$ denotes a semantic distance metric in the image embedding space. Conversely, for non-members, the expectation of this distance grows as the model’s conditional distribution reacts more sensitively to changes in $c$.
% This stability can also be captured by analyzing the cross-modal similarity gradient:
% \begin{equation}
% \frac{\partial}{\partial \delta_c}
% d\big(\mathcal{E}v(x), \mathcal{E}v(\hat{x}_{c^{'}})\big)
% \approx 0
% \quad \text{if} \quad x \in \mathcal{D}_t,
% \end{equation}
% implying that textual perturbations induce negligible changes in the generated visual semantics for member samples~\cite{somepalli2023diffusion}.
% In essence, membership correlates with both lower conditional entropy and higher cross-modal stability, which provides the theoretical foundation for our proposed method.
% This theoretical insight motivates the design of our proposed \textbf{SD-MIA} framework, which probes diffusion models through controlled cross-modal perturbations to measure their semantic response sensitivity. By quantifying how invariant the generated image remains under textual variations, we extract a discriminative signal reflecting the model’s internal memorization strength for each text–image pair.

% 1. 对suspected 图片的描述进行扰动（如果没有自带的描述，则使用多模态大模型生成。）扰动方式有 a. 重写（保持语义和风格） b. 对风格扰动（保持语义） c. 对语义扰动（保持风格）。 2. 使用target 模型对扰动后的描述生成image(n次) 3. 计算clip(原描述) concat clip(原图)  与  clip(扰动描述) concat clip(生成的图) 之间相似度。取top-k 。 4将三种扰动方式结合计算score 相似度越大，越有可能在pretraining过程中出现过。
\subsection{Perturbation-Guided SD-MIA Framework}

The proposed SD-MIA framework leverages the cross-modal consistency to infer pretraining-data membership under a black-box setting. 
The key insight is that the degree of visual stability in response to textual perturbations encodes the strength of the model’s internal text–image alignment learned during pre-training.
The overall workflow of the proposed method is illustrated in Figure~\ref{fig:method}. 
Given a suspected image $x$ and corresponding semantic description $c$, we first propose a vision-aware description perturbation method to
construct a set of perturbations from visual semantics or visual style.
Each perturbed description is then used to query the target diffusion model $\mathcal{M}_\theta$, yielding a collection of synthetic images.
Next, we measure cross-modal consistency between each synthetic image and the suspected image in both visual and textual feature spaces to capture fine-grained memorization signals.
To mitigate sampling variance, the generation process is repeated multiple times per perturbation. We introduce a MAX-$k\%$ selection mechanism to emphasize the most stable model responses, which are most indicative of memorization.
Finally, we introduce an aggregation strategy across perturbation types to form the decision statistic for membership inference, effectively quantifying how robustly the diffusion model reproduces $x$ under controlled textual variations.


\subsection{Vision-Aware Description Perturbation}


The first stage of the SD-MIA framework constructs a controlled set of caption perturbations tailored to the visual content of the suspected image. Given an associated description $c$ (or an LMM-generated one when unavailable), we generate a perturbation set
$\mathcal{C}(c) = \{c^{(1)}, c^{(2)}, \dots, c^{(M)}\}$, where each $c^{(i)}$ is produced under a distinct, vision-aware perturbation strategy. Unlike purely text-based paraphrasing, our design explicitly conditions perturbations on the visual characteristics of $x$, ensuring that the modified captions remain grounded in the underlying image semantics or style. To ensure the perturbations maintain content integrity and fluency, we employ a LLM (e.g. GPT-5) to construct linguistically diverse descriptions while preserving cross-modal consistency.
These perturbations are created via three vision-aware strategies:
\begin{enumerate}

    \item \textbf{Paraphrase Perturbation:} Rewrites the description while preserving both the semantic content and the visual style of the corresponding image.
    This perturbation introduces lexical and syntactic variation and primarily probes  the robustness of the model’s cross-modal alignment to subtle, vision-consistent textual changes.

    \item \textbf{Visual Style Perturbation:} 
    % This perturbation modifies visual stylistic attributes implied by the suspected image while preserving semantic content the original description intact. 
    Modifies stylistic elements of the description that affect the generated image’s visual style attributes, while retaining the original semantic content. 
    This perturbation reveals how much the visual rendering depends on style cues versus semantic understanding, and highlighting sensitivity to stylistic variations in the generation process.
    % This perturbation is particularly useful for probing the model's ability to disentangle semantic content from visual representation in the generation process.
    \item \textbf{Visual Semantic Perturbation:} Alters the semantic content of the description while maintaining the visual style of the suspected image. 
    This perturbation explicitly evaluates how strongly the target model anchors its generated image to the original semantic content.
    
\end{enumerate}
These vision-aware strategies collectively enable a comprehensive assessment of the model's text–image alignment under controlled variations. 

% target different aspects of the model's text–image alignment, enabling a comprehensive analysis of how the model handles variations in textual input. 
% The perturbations are crafted to explore the limits of the model’s robustness to semantic and visual shifts, which provides valuable insights into its internal cross-modal memorization and generalization behavior.

To ensure that the perturbations do not deviate significantly from the original description, we enforce a consistency constraint that requires the generated content to maintain high semantic similarity to the original description. Specifically, for each perturbation $c^{(i)}$, we impose the following constraint:
\[
\mathrm{sim}\left( \mathcal{E}_t(c^{(i)}), \mathcal{E}_t(c) \right) \geq \tau_t,
\]
where $\mathcal{E}_t(\cdot)$ denotes the text encoder (e.g., CLIP’s text encoder), and $\tau_t$ is a threshold that ensures that the perturbation does not deviate too far from the original description in terms of its semantic content.


\subsection{Memorization-Sensitive Generation Dynamics}
After generating the perturbed descriptions, we query the target diffusion model $\mathcal{M}_\theta$ to obtain corresponding synthetic images. For each perturbed caption $c^{(i)}$, we generate multiple independent samples:
\begin{equation}
\hat{x}_{c^{(i)}}^{(j)} \sim p_\theta(\cdot \mid c^{(i)}), \quad j = 1, \dots, N,
\end{equation}
where $p_\theta$ denotes the conditional generative distribution parameterized by the learned score function $\nabla_x \log p_t(x_t \mid c)$. During the denoising trajectory, the model iteratively refines the latent variable via:
\begin{equation}
x_{t-1} = x_t + \Delta_t \nabla_x \log p_t(x_t \mid c),
\end{equation}  
gradually restoring the image conditioned on textual description.
Then we leverage explicit analyze of generation dynamics across repeated samplings. By examining how the model responds to identical perturbed prompts across multiple stochastic denoising trajectories, we expose memorization-sensitive behavior that is otherwise hidden in single-sample evaluations. For member pairs $(x,c)$, the learned score field exhibits locally stable gradient flows, which suppress variability in generated outputs even under perturbed textual conditions. This stability yields a bounded perceptual drift:
\begin{equation}
\mathbb{E}_{j} \Big[ d(\mathcal{E}_v(\hat{x}_{c^{(i)}}^{(j)}), \mathcal{E}_v(x)) \Big] \leq \varepsilon,
\end{equation}
where $\mathcal{E}_v$ denotes the image encoder and $d(\cdot, \cdot)$ a semantic distance metric. In contrast, non-member pairs show higher sensitivity, with the conditional distribution producing more diverse outputs under the same perturbations.

% By explicitly analyzing the distribution and stability of generated samples rather than relying on a single reconstruction, we introduce a principled approach to quantify memorization-induced invariance in diffusion models. This enables a more reliable signal for membership inference.
% capturing both the mean alignment and the variance of responses across multiple generations.


% \subsection{Diffusion Model Response Analysis}
% After generating the perturbed descriptions, we perform end-to-end queries to the target diffusion model $\mathcal{M}_\theta$ under the black-box setting to obtain the corresponding synthesized images. Specifically, for each perturbed description $c^{(i)}$, the model generates:
% \begin{equation}
% \hat{x}_{c^{(i)}} \sim p_\theta(\cdot \mid c^{(i)}),
% \end{equation}
% where $p_\theta$ denotes the conditional generative distribution parameterized by the learned score function $\nabla_x \log p_t(x_t \mid c)$.
% During the denoising trajectory, the model iteratively refines the latent variable via:
% \begin{equation}
% x_{t-1} = x_t + \Delta_t \nabla_x \log p_t(x_t \mid c),
% \end{equation}
% gradually restoring the image conditioned on textual description.  
% If $(x, c)$ was part of the training distribution, the learned score field exhibits locally consistent gradient flows, leading to nearly invariant reconstructions under small perturbations of $c$.  
% Formally, the expected perceptual drift satisfies:
% \begin{equation}
% \mathbb{E}_{x' \sim p_\theta(\cdot \mid c^{i})}
% \Big[
% d(\mathcal{E}_v(x'), \mathcal{E}_v(x))
% \Big]
% \leq \varepsilon,
% \end{equation}
% where $d(\cdot,\cdot)$ denotes a semantic distance metric in the image embedding space. $ \mathcal{E}_v$ is the image encoder.
% Non-member pairs, in contrast, yield higher sensitivity as the conditional distribution reacts more strongly to textual perturbations.


\subsection{Cross-Modal Consistency Scoring}
After obtaining the perturbed descriptions and corresponding generated samples, we estimate the cross-modal consistency between the original pair $(x,c)$ and each perturbed pair $\big(\hat{x}_{c^{(i)}}, c^{(i)}\big)$. The goal is to quantify how strongly the diffusion model preserves the joint text–image relationship when subjected to controlled perturbations, a signal that directly reflects potential memorization.
For each candidate instance, we compute the joint embeddings of the original description–image pair and each perturbed pair:
\[
z = \mathcal{E}_t(c) \oplus \mathcal{E}_v(x), \qquad 
z_{c^{(i)}}^{(j)} = \mathcal{E}_t(c^{(i)}) \oplus \mathcal{E}_v\big(\hat{x}_{c^{(i)}}^{(j)}\big),
\]
where $\oplus$ denotes vector concatenation, and $\mathcal{E}_t$ and $\mathcal{E}_v$ represent the text and image encoders. Concatenation ensures that semantic and visual alignment are evaluated jointly rather than as decoupled modalities. We compute a similarity score for each perturbed sample:
\begin{equation}
S_{c^{(i)}}^{(j)}
=
F\!\left(z,\,
z_{c^{(i)}}^{(j)}\right),
\end{equation}
where $F$ is a similarity metric such as cosine similarity.

Since diffusion models exhibit stochastic variability across generations, the distribution of $\{S_{c^{(i)}}^{(j)}\}_{j=1}^{n}$ carries valuable information about memorization-induced stability. To exploit this, we introduce a \emph{MAX-$k\%$ selection} strategy that focuses on the most consistent outputs:
% \begin{equation}
% S_{c^{(i)}}^{K}
% = \frac{1}{\left \lfloor n*K\%  \right \rfloor }\text{Max-}k\%\big(S_{c^{(i)}}^{(1)},\dots,S_{c^{(i)}}^{(n)}\big),
% \end{equation}
\begin{equation}
S_{c^{(i)}}^{K}
=
\frac{1}{n}
\sum_{j=1}^{n}
S_{c^{(i)}}^{(j)\!\uparrow},
\qquad 
n = \left\lfloor N \cdot K\% \right\rfloor ,
\end{equation}
which computes the average of the top $K\%$ largest similarity values. This selection acts as a min–max style estimator: it suppresses noise from low-quality or highly variable generations while emphasizing the most stable responses, which are most indicative of membership.

Finally, the aggregated consistency score across perturbation strategies is defined as
\begin{equation}
S = \Psi\big(S_{c^{(1)}}^{K}, S_{c^{(2)}}^{K}, S_{c^{(3)}}^{K}\big),
\end{equation}
where $\Psi$ is an aggregation function such as linear combination. A sample is classified as a member if $S$ exceeds a decision threshold.  
This cross-modal consistency measure provides a robust and discriminative indicator of whether the diffusion model internally anchors to the suspected sample, thereby revealing memorization behavior.



% After generating the perturbed description and corresponding images, we proceed to estimate the cross-modal consistency between the textual descriptions and the generated images. The key objective of this stage is to measure the alignment between the original and perturbed descriptions and their corresponding images, using both textual and visual embeddings. This step plays a crucial role in inferring whether the suspected image might have been part of the pretraining dataset of the target model.

% For each suspected image \( x \), we compute the embeddings of the original description \( c \) and image \( x \), and the embeddings of each perturbed description \( c^{(i)} \) and the generated image \( \hat{x}_{c^{(i)}} \):

% \[
% \mathcal{E}_t(c) \oplus \mathcal{E}_v(x), \quad \mathcal{E}_t(c^{(i)}) \oplus \mathcal{E}_v(\hat{x}_{c^{(i)}}),
% \]

% where \( \oplus \) denotes the concatenation of the textual and visual embeddings, and \( \mathcal{E}_t \) and \( \mathcal{E}_v \) are the text and image encoders, respectively.

% We define the consistency score $S$ by computing the similarity between the concatenated embeddings of the original description-image pair and the perturbed description-generated image pair:
% \begin{equation}
%     S_{c^{i}} = F \left( \mathcal{E}_t(c) \oplus \mathcal{E}_v(x), \mathcal{E}_t(c^{(i)}) \oplus \mathcal{E}_v(\hat{x}_{c^{(i)}}) \right),
% \end{equation}
% where $F$ denotes the function to measure similarity (e.g. cosine).
% The rationale for using concatenated embeddings is to capture both the semantic alignment and the visual consistency between the description and the generated image. By concatenating both text and image embeddings, we ensure a joint evaluation of their relationship, rather than treating them independently.



% In order to account for the inherent variability in generated images, we propose a Max-K\% selection strategy. This allows us to mitigate the influence of outliers or extreme values in the similarity distribution and ensures that our consistency measure is not overly sensitive to one-off cases. 
% Specifically,
% we aggregate the Max-K\% consistency score from multiple generated images for each perturbation \( c^{(i)} \). 
% Formally, the Max-K\% consistency $S_{c^{i}}^{K}$ for each perturbation \( c^{(i)} \) are selected as: $S_{c^{i}}^{K} = Max-K\% (S_{c^{i}}^{1}, S_{c^{i}}^{2}, S_{c^{i}}^{3}, \cdots, S_{c^{i}}^{N}), $
% where \( n \) is the number of generated images for each perturbation, and \( \text{Top-k} \) selects the \( k \) largest similarity values. This strategy ensures that we focus on the most consistent generated images, providing a more stable evaluation of cross-modal alignment.

% The final consistency score $S_{c}$ is aggregated by the Max-K\% consistency scores across all three perturbation strategies.
% Finally, if $S_{c}$ exceeds a predefined threshold, we classify the suspected image as a member of the pretraining dataset. Otherwise, it is classified as a non-member.
% This approach provides a robust measure of cross-modal consistency, enabling us to infer the likelihood of an image being part of the model's pretraining data based on its similarity to perturbed descriptions and generated images.




